From Small Space to Small Width in Resolution

In 2003, Atserias and Dalmau resolved a major open question about the resolution proof system by establishing that the space complexity of CNF formulas is always an upper bound on the width needed to refute them. Their proof is beautiful but somewhat mysterious in that it relies heavily on tools from finite model theory. We give an alternative, completely elementary proof that works by simple syntactic manipulations of resolution refutations. As a by-product, we develop a "black-box" technique for proving space lower bounds via a "static" complexity measure that works against any resolution refutation---previous techniques have been inherently adaptive. We conclude by showing that the related question for polynomial calculus (i.e., whether space is an upper bound on degree) seems unlikely to be resolvable by similar methods.

==> figPebblingFormula1.tex <==
%%%
%%%  O B S O L E T E
%%%
\ifthenelse{\boolean{conferenceversion}}
{\begin{figure*}[tp]}
{\begin{figure}[tp]}
  \subfigure
  [Pyramid graph $\Pi_2$ of height 2.]
  {
    \label{fig:pebbling-contradiction-for-Pi-2-graph}
    \begin{minipage}[b]{0.40\linewidth}
      \centering
      \includegraphics{smallPyramidHeight2.1}%
    \end{minipage}
  }
  \hfill
  \subfigure
  [Pebbling contradiction
    {$\pebcontr[{\pyramidgraph[2]}]{}$}.%
%        {$\pebcontr[\Pi_2]{}$}.%
  ]
  {
    \label{fig:pebbling-contradiction-for-Pi-2-Peb1}
    \begin{minipage}[b]{0.55\linewidth}
      \centering
      \begin{gather*}
	\begin{aligned}
	  &
	  u
	  \\
	  \land \
	  &v
	  \\
	  \land \
	  &w
	  \\
	  \land \
	  &(\olnot{u} \lor \olnot{v} \lor x)
	  \\
	  \land \
	  &(\olnot{v} \lor \olnot{w} \lor y)
	  \\
	  \land \
	  &(\olnot{x} \lor \olnot{y} \lor z)
	  \\
	  \land \
	  &\olnot{z}
	\end{aligned}
      \end{gather*}
    \end{minipage}
  }

  \subfigure[Bottom-up refutation of {$\pebcontr[{\pyramidgraph[2]}]{}$}.]{
  \label{fig:pebbling-contradiction-for-Pi-2-bottom-up}
  \begin{minipage}[b]{0.4\linewidth}
    \begin{flagderiv}
      \step{bdlu}{u}{Axiom}
      \step{bdlv}{v}{Axiom}
      \step{bdluvx}{\olnot{u} \lor \olnot{v} \lor x}{Axiom}
      \step{bresvx}{\olnot{v} \lor x}{Resolve \ref{bdlu} \ref{bdluvx}}
      \step{bresx}{x}{Resolve \ref{bdlv} \ref{bresvx}}
      \step{bdlw}{w}{Axiom}
      \step{bdlvwy}{\olnot{v} \lor \olnot{w} \lor y}{Axiom}
      \step{breswy}{\olnot{w} \lor y}{Resolve \ref{bdlv} \ref{bdlvwy}}
      \step{bresy}{y}{Resolve \ref{bdlw} \ref{breswy}}
      \step{bdlxyz}{\olnot{x} \lor \olnot{y} \lor z}{Axiom}
      \step{bresyz}{\olnot{y} \lor z}{Resolve \ref{bresx} \ref{bdlxyz}}
      \step{bresz}{z}{Resolve \ref{bresy} \ref{bresyz}}
      \step{bdlz}{\olnot{z}}{Axiom}
      \step{bres}{\bot}{Resolve \ref{bresz} \ref{bdlz}}
    \end{flagderiv}
  \end{minipage}
  }
  \hfill
  \subfigure[Top-down refutation of {$\pebcontr[{\pyramidgraph[2]}]{}$}.]{
  \label{fig:pebbling-contradiction-for-Pi-2-top-down}
  \begin{minipage}[b]{0.55\linewidth}
   \hspace{0.15\linewidth}
   \begin{minipage}[b]{0.4\linewidth}
    \begin{flagderiv}
      \step{tdlz}{\olnot{z}}{Axiom}
      \step{tdlxyz}{\olnot{x} \lor \olnot{y} \lor z}{Axiom}
      \step{tresxy}{\olnot{x} \lor \olnot{y}}{Resolve \ref{tdlz} \ref{tdlxyz}}
      \step{tdlvwy}{\olnot{v} \lor \olnot{w} \lor y}{Axiom}
      \step{tresvwx}{\olnot{v} \lor \olnot{w} \lor \olnot{x}}{Resolve \ref{tresxy} \ref{tdlvwy}}
      \step{tdlw}{w}{Axiom}
      \step{tresvx}{\olnot{v} \lor \olnot{x}}{Resolve \ref{tresvwx} \ref{tdlw}}
      \step{tdluvx}{\olnot{u} \lor \olnot{v} \lor x}{Axiom}
      \step{tresuv}{\olnot{u} \lor \olnot{v}}{Resolve \ref{tresvx} \ref{tdluvx}}
      \step{tdlv}{v}{Axiom}
      \step{tresu}{\olnot{u}}{Resolve \ref{tresuv} \ref{tdlv}}
      \step{tdlu}{u}{Axiom}
      \step{tres}{\bot}{Resolve \ref{tresu} \ref{tdlu}}
    \end{flagderiv}
   \end{minipage}
  \end{minipage}
  }
  \caption{Pebbling contradiction
%        $\pebcontr[{\pyramidgraph[2]}]{}$
    for the pyramid graph
    $\pyramidgraph[2]$
    with example resolution refutations.
%        $\Pi_2$.
%        of height~$2$.
  }
  \label{fig:pebbling-contradiction-for-Pi-2}
\ifthenelse{\boolean{conferenceversion}}
{\end{figure*}}
{\end{figure}}



==> figRefutations.tex <==
%%%
%%% When put in a separate figure, the flagderiv refutations screw up
%%% the horizontal spacing in a *major* way... -JN
%%%
\begin{figure}[t]
  \subfigure[Bottom-up refutation of {$\pebcontr[{\pyramidgraph[2]}]{}$}.]{
  \label{fig:pebbling-contradiction-for-Pi-2-bottom-up}
  \begin{minipage}[b]{0.4\linewidth}
    \begin{flagderiv}
      \step{bdlu}{u}{Axiom}     
      \step{bdlv}{v}{Axiom}
      \step{bdluvx}{\olnot{u} \lor \olnot{v} \lor x}{Axiom}
      \step{bresvx}{\olnot{v} \lor x}{Resolve \ref{bdlu} \ref{bdluvx}}
      \step{bresx}{x}{Resolve \ref{bdlv} \ref{bresvx}}
      \step{bdlw}{w}{Axiom}
      \step{bdlvwy}{\olnot{v} \lor \olnot{w} \lor y}{Axiom}
      \step{breswy}{\olnot{w} \lor y}{Resolve \ref{bdlv} \ref{bdlvwy}}
      \step{bresy}{y}{Resolve \ref{bdlw} \ref{breswy}}
      \step{bdlxyz}{\olnot{x} \lor \olnot{y} \lor z}{Axiom}
      \step{bresyz}{\olnot{y} \lor z}{Resolve \ref{bresx} \ref{bdlxyz}}
      \step{bresz}{z}{Resolve \ref{bresy} \ref{bresyz}}
      \step{bdlz}{\olnot{z}}{Axiom}
      \step{bres}{\bot}{Resolve \ref{bresz} \ref{bdlz}}
    \end{flagderiv}
  \end{minipage}
  }
  \hfill
  \subfigure[Top-down refutation of {$\pebcontr[{\pyramidgraph[2]}]{}$}.]{
  \label{fig:pebbling-contradiction-for-Pi-2-top-down}
%      \begin{minipage}[b]{0.55\linewidth}
%       \hspace{0.15\linewidth}
   \begin{minipage}[b]{0.4\linewidth}
    \begin{flagderiv}
      \step{tdlz}{\olnot{z}}{Axiom}
      \step{tdlxyz}{\olnot{x} \lor \olnot{y} \lor z}{Axiom}
      \step{tresxy}{\olnot{x} \lor \olnot{y}}{Resolve \ref{tdlz} \ref{tdlxyz}}
      \step{tdlvwy}{\olnot{v} \lor \olnot{w} \lor y}{Axiom}
      \step{tresvwx}{\olnot{v} \lor \olnot{w} \lor \olnot{x}}{Resolve \ref{tresxy} \ref{tdlvwy}}
      \step{tdlw}{w}{Axiom}
      \step{tresvx}{\olnot{v} \lor \olnot{x}}{Resolve \ref{tresvwx} \ref{tdlw}}
      \step{tdluvx}{\olnot{u} \lor \olnot{v} \lor x}{Axiom}
      \step{tresuv}{\olnot{u} \lor \olnot{v}}{Resolve \ref{tresvx} \ref{tdluvx}}
      \step{tdlv}{v}{Axiom}
      \step{tresu}{\olnot{u}}{Resolve \ref{tresuv} \ref{tdlv}}
      \step{tdlu}{u}{Axiom}
      \step{tres}{\bot}{Resolve \ref{tresu} \ref{tdlu}}
    \end{flagderiv}
   \end{minipage}
%      \end{minipage}
  }
  \caption{Example resolution refutations of
    $\pebcontr[{\pyramidgraph[2]}]{}$.
  }
  \label{fig:pebbling-contradiction-for-Pi-2-refutations}
\end{figure}



